Linguistic Profiling of Deepfakes: An Open Database for Next-Generation Deepfake Detection

The emergence of text-to-image generative models has revolutionized the field of deepfakes, enabling the creation of realistic and convincing visual content directly from textual descriptions. However, this advancement presents considerably greater challenges in detecting the authenticity of such content. Existing deepfake detection datasets and methods often fall short in effectively capturing the extensive range of emerging deepfakes and offering satisfactory explanatory information for detection. To address the significant issue, this paper introduces a deepfake database (DFLIP-3K) for the development of convincing and explainable deepfake detection. It encompasses about 300K diverse deepfake samples from approximately 3K generative models, which boasts the largest number of deepfake models in the literature. Moreover, it collects around 190K linguistic footprints of these deepfakes. The two distinguished features enable DFLIP-3K to develop a benchmark that promotes progress in linguistic profiling of deepfakes, which includes three sub-tasks namely deepfake detection, model identification, and prompt prediction. The deepfake model and prompt are two essential components of each deepfake, and thus dissecting them linguistically allows for an invaluable exploration of trustworthy and interpretable evidence in deepfake detection, which we believe is the key for the next-generation deepfake detection. Furthermore, DFLIP-3K is envisioned as an open database that fosters transparency and encourages collaborative efforts to further enhance its growth. Our extensive experiments on the developed benchmark verify that our DFLIP-3K database is capable of serving as a standardized resource for evaluating and comparing linguistic-based deepfake detection, identification, and prompt prediction techniques.

==> backup/01_intro_backup_20230607.tex <==
\section{Introduction}

% \zhiwu{@Yabin, we could consider the following logic:  Part 1. New challenge: traditional deepfakes -> prompted deepfakes (refer to the paper '' and ''. 
% Part 2. New approach: from detection to dissection of deepfakes, Part 3. Summary of our contributions}
% ZH: the following drafted introduction is merely for a reference and could be furhter improved...


The field of deepfakes has experienced a significant shift in recent years, moving beyond traditional generative models focused on realistic images and videos to the emergence of text-to-image (T2I) generative models. These new models have unlocked new possibilities for creating highly realistic and convincing deepfakes. Early deepfakes were generated using conventional generative models like  generative adversarial networks (GANs) \cite{goodfellow2020generative, arjovsky2017wasserstein, karras2019style} and variational autoencoders (VAEs) \cite{tolstikhin2017wasserstein, hinton2011transforming}, which learned patterns from large datasets to modify existing visuals by swapping faces, altering expressions, or creating fabricated scenes. Recent text-to-image generative models like DALL·E \cite{ramesh2022hierarchical}, Imagen \cite{saharia2022photorealistic} and Stable Diffusion \cite{rombach2021highresolution} have revolutionized deepfakes by enabling the direct synthesis of images from textual descriptions or prompts. 

The emergence of text-to-image generative models has brought about exciting opportunities in a wide range of domains. Artists, designers, and content creators can now quickly visualize their ideas by providing textual prompts, eliminating the need for manual image manipulation. Furthermore, these models have found applications in virtual reality, gaming, and storytelling, allowing text-based descriptions to be transformed into immersive visual experiences. However, the proliferation of text-to-image generative models also raises serious ethical concerns. The potential for misuse and the spread of misleading or false information raises concerns regarding the authenticity and trustworthiness of visual content. 



\begin{figure}[t]
\begin{floatrow}
\ffigbox{%
  \centering
  \includegraphics[width=0.44\textwidth]{Figs/dflip_overview.pdf}%
}{%
% \zhiwu{'Deepfak?' The content in 'Profile' box can be further aligned.}
  \caption{DFLIP-3K enables linguistic profiling of deepfakes, including the assessment of authenticity (deepfake detection), the identification of source model (deepfake identification), and the prediction of source prompt (prompt prediction).}%
  \label{fig:dflip_overview}
}
\capbtabbox{%
\centering
        \begin{footnotesize}
        \resizebox{0.92\linewidth}{!}{
        \begin{tabular}{ccc}\hline
        \textbf{Dataset}  & \textbf{\# Generative Models} \\
        \hline
        \multicolumn{2}{c}{\textbf{Early Datasets}}         \\ \hline
        FaceForensic++ \cite{rossler2019faceforensics++}  &  4 \\
        DFDC \cite{dolhansky2020deepfake}      & 8 \\

        % Celab-DF v2 \cite{} & \\
        % WhichFaceReal \cite{}    & \\
        WildDeepfake \cite{zi2020wilddeepfake}  & Unknown \\
        % CNNfake \cite{}     &                        \\
        % GANfake \cite{}  &   \\
        CDDB \cite{li2022continual}  &  11 \\
       \hline
        \multicolumn{2}{c}{\textbf{Recent Datasets}}         \\ \hline
        DiffusionDB \cite{wang2022diffusiondb} &    1 \\
        SAC \cite{pressmancrowson2022}    &    4   \\
        Pick-a-Pic \cite{kirstain2023pick}    &   2 \\ 
        HP \cite{wu2023better}    &    1 \\
        MidJourney(250K) \cite{turc2023midjourney}     &   Unknown \\ 
        \textbf{DFLIP-3K (Ours)} & \textbf{$\approx$ 3K }                    \\
          \hline
        \end{tabular}
        }
        \end{footnotesize}
}{%
% 
  \caption{A comparison of DFLIP-3K against the early and recent deepfake datasets. It collects deepfakes from about 3K generative models, representing the largest scale in terms of the number of deepfake models.}%
  \label{tab:deepfake_databases}
}
% \zhiwu{We could put the full table in the suppl.}
\end{floatrow}
\vspace{-0.5cm}
\end{figure}


In this context, this paper introduces an open database (DFLIP-3K) for linguistic profiling of deepfakes, which aims at \XPDel{deriving}\XP{the} next-generation deepfake detection. The proposed database addresses the need for standardized resources that focus on analyzing the linguistic characteristics of deepfake content. By incorporating linguistic analysis into the detection process, as showcased in Fig.\ref{fig:dflip_overview}, the objective of this benchmark database is to advance \emph{the detection of deepfakes, the identification of deepfake source models (i.e., deepfake copyright), as well as the prediction of textual prompts} that are used for text-to-image generation. 
In other words, this database aims to promote the field of deepfake detection by enabling the development of robust algorithms that consider the unique linguistic footprints left by text-driven deepfakes. This provides researchers and practitioners with a common standard for evaluating and comparing their linguistic-based deepfake detection techniques. 

In particular, the established DFLIP-3K database encompasses approximately 300K deepfake samples produced from about 3K generative models, which is the largest scale in the literature of deepfake detection. In addition, we gather about \zhiwu{170K} textual prompts that are used to create images. The collected prompts allow for the exploitation of linguistic profiling in simultaneous deepfake detection, identification, and prompt prediction. 
% \XP{[this sentence shall be further polished]}..
Apart from curating this database, we thoroughly examine the ethical considerations and potential flaws associated with large-scale data collection. By making DFILP-3K publicly available, we provide the community with the initial opportunity to further enhance a database of such application and magnitude. 
% \XP{[it appears to me that the focus is on the size.]}


To assess the potential value of DFLIP-3K, we establish a benchmark for linguistic profiling in simultaneous deepfake detection, identification, and prompt prediction. Based on this benchmark, we conduct several experiments. Our evaluation focuses on three state-of-the-art vision-language models adapted for deepfake profiling. The results reveal that these vision-language models outperformed traditional vision models in detecting and identifying deepfakes. Unlike vision-based models, our suggested vision-language models have the ability to generate either regular image captions or textual prompts in specific formats for image generation. The evaluations demonstrate that training the vision-language models with our collected prompts leads to more sensible prompt prediction, resulting in generated images that closely resemble the input deepfake images in terms of perceptual, semantic, and aesthetic similarities. Furthermore, we also show that the suggested deepfake profiling facilitates the interpretability of the generated content using generative models.

Despite the validation results, DFLIP-3K is not considered a finalized data product at this stage. Given the continuous emergence of generative models, the comprehensive curation of DFLIP-3K for widespread usage extends beyond the scope of a single research paper. Therefore, in addition to releasing the dataset, we are also sharing the software stack that we developed for assembling DFLIP-3K. We consider this initial data release and accompanying paper as an initial step towards creating a widely applicable deepfake dataset suitable for a broader range of linguistic profiling tasks. Consequently, we are making all collection methods, metadata, and deepfake data within our database openly accessible to fully unleash its potential for next-generation deepfake detection.


\begin{comment}
%ZH: original version

In particular, the established database encompasses diverse deepfake samples generated by \emph{15 text-to-image generation models?}, most of which are collected along with linguistic features (textual prompts) that are utilized by users for text-to-image deepfake generation...@Yabin, we could present key features of our database here...

In summary, the key contribution of this paper is to explore the construction and characteristics of the proposed database, emphasizing its significance in advancing deepfake detection through linguistic profiling. Additionally, it discusses the applications and challenges associated with linguistic-based detection methods, highlighting the importance of integrating linguistic analysis into the broader framework of deepfake detection. By harnessing the power of linguistics, researchers can strive to stay ahead of evolving deepfake techniques, safeguarding the integrity of digital media, and preserving trust in an increasingly interconnected world. 
\end{comment}

==> dataset.tex <==

\section{Benchmark Experiments and Results}
In this section, we present our experimental setup along with the detailed training procedures. 
We report the performance of several baseline methods and discuss limitations.

\subsection{Benchmark Description}

We can address three critical tasks of deepfake detection using the proposed DFLIP dataset once for all: Deepfake Detection, Copyright Identification, and Image2Prompt Generation. 
Thus we present three different versions of the benchmark, as follows:

\begin{itemize}
\item Deepfake Detection: detecting fake images generated by T2I techniques;
\item Copyright Identification: identifying which deepfake model generates the image;
\item Image2Prompt Generation: Generating prompts given reference images.
\end{itemize}

Detecting deepfakes is a fundamental task for our database, especially given recent breakthroughs in large-scale text-to-image (T2I) generative models that provide individuals with more opportunities to create high-quality deepfakes. As deepfakes blur the line between reality and fantasy, distinguishing them from traditional art becomes increasingly challenging. 

It is also essential to detect whether a given image is a deepfake and which deepfake model is used to generate the image.
This can help model publishers protect their models.
However, identifying the origins of deepfakes is a non-trivial task due to their high diversity and the prevalence of customized models trained on private data. 

Furthermore, the Image2Prompt Generation problem has emerged due to recent developments in T2I models. By training generative models on prompts, we can generate high-quality images and gain a deeper understanding of the underlying mechanisms behind T2I deepfake generation.


\subsection{Baselines}
Deepfake detection and copyright identification are typical binary and multi-classification tasks, respectively. For these tasks, we can employ conventional classification networks as our baseline models. Additionally, for deepfake detection, we apply the state-of-the-art deepfake CNN detector, CNNDet, as our baseline model.
Regarding image-to-prompt generation, this is a recently emerging task for which there are no dedicated methods available yet. Therefore, we choose mainstream image captioning methods as our baseline models.

Traditionally, we have to train separate networks for each task. 
However, with the recent development of multimodal language models, we can ensemble deepfake detection, copyright identification, and prompt generation by training a single language model. To this end, we utilize Flamingo, a multimodal language model that leverages pre-trained vision and language models to accept images and text as input and generate free-form text as output. We incorporate Flamingo into our database to perform these tasks.

We opt to use the OpenFlamingo 9B implementation, which is trained on large multimodal datasets, such as Multimodal C4 and LAION-2B. This model uses a CLIP ViT-Large vision encoder and a LLaMA-7B language model, and it incorporates cross-attention layers into the language model to combine these two modalities. We further fine-tune the model on our DFLIP datasets.


\subsection{Metrics}
We use three primary evaluation metrics in the DFLIP database, namely average detection accuracy (AA), copyright identification accuracy (CA), and prompt generation quality (PGQ).

Following previous works~\cite{wang2020cnn}, we propose to use two average detection accuracy metrics: the task-agnostic average detection accuracy (TAAA) and the task-wise average detection accuracy (TWAA).
TAAA calculates the test accuracy of all samples. However, this metric may overlook the accuracy of deepfake methods with fewer test samples.
As an alternative, TWAA can be computed as follows:

\begin{equation}
AA=\frac{1}{n}\sum_{i=1}^{n}B_{n},
\label{eq:aa}
\end{equation}

where $B_{i}$ represents the test accuracy of the $i$-th deepfake model, and $n$ is the total number of deepfake methods. This metric provides a better evaluation of the overall performance of the detector.

In terms of copyright identification, we suggest further reporting the copyright identification accuracy (CA), which calculates the accuracy of classifying images into the correct deepfake models. The calculation of the copyright identification accuracy (CA) is:

\begin{equation}
CA = \frac{N^{TP}{deepfakes}+N^{TN}{real}}{N_{total}},
\label{eq:ca}
\end{equation}

where $N^{TP}{deepfakes}$ represents the true positives of deepfakes classified as their corresponding generators, and $N^{TN}{real}$ represents the true negatives of real images classified correctly. $N_{total}$ denotes the total number of test samples. All real images are classified as a single class in the CA calculation.

To evaluate the quality of generated images, we consider two aspects. First, we calculate the average cosine similarity between CLIP embeddings of the generated images and the reference images used to generate the prompts to evaluate the image alignment quality. This metric is referred to as CLIP-ImgSim. Second, we use the Learned Perceptual Image Patch Similarity (LPIPS) to judge the perceptual similarity between two images. Additionally, to generate better images, we also incorporate aesthetic scores. We use the LAION-Aesthetic detector to calculate the average aesthetic score of the generated images for different prompt generation methods. We generate ten images using different random seeds for each prompt and calculate their CLIP-ImgSim and LPIPS scores, as well as their aesthetic scores.


To train models, we require a sufficiently large dataset of deepfake images. Therefore, we need to further filter the dataset to ensure that all methods have at least 200 images for training and 50 images for testing. 
This is mainly due to the fact that most personalized diffusion methods have fewer than ten images, which are insufficient for training. The processed dataset is presented in the table. 
Additionally, we have cleaned up the prompts of the personalized diffusion methods' images, removing many special characters and retaining only commas. Although this may not fully capture the original prompts' effects, it is a more standardized format that is easier to train.

During training, we use ResNet-50 as the backbone for CNNDet, which is pre-trained on ImageNet. We fine-tune ResNet-50 on ProGAN for ODD. To train CNNDet on Stable Diffusion, we also use the suggested data augmentation methods of Blur+JPEG. Moreover, we introduce ViT-B/16 as an enhanced deepfake detector by replacing ResNet-50 and pre-training it on ImageNet. We employ our suggested fine-tuning and prompt-tuning strategies to further improve its performance. All methods are implemented using their original hyper-parameters.

For prompts generation during testing, we randomly sample 1,000 images from the test set as reference images. We then use our model to predict the prompts or captions for these images. We input the output prompts into the WebUI to generate ten images.






\begin{table}[]
\begin{tabular}{lrrrrrrrrr}
\hline
\multicolumn{1}{c}{} & \multicolumn{6}{c}{Deepfake Models} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ \cline{2-7}
\multicolumn{1}{c}{\multirow{-2}{*}{Methods}} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{PD} & \multicolumn{1}{c}{DALLE} & \multicolumn{1}{c}{MJ} & \multicolumn{1}{c}{Imagen} & \multicolumn{1}{c}{Parti} & \multicolumn{1}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Task-agnostic \\ AA\end{tabular}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Task-wise \\ AA\end{tabular}}} & \multicolumn{1}{c}{\multirow{-2}{*}{F1}} \\ \hline
ResNet${^*}$ \cite{?} & 1 & & & & & & & & \\
ViT${^*}$ \cite{?}  & 64.50 & 84.01 & 80.15 & 77.54 & 72.58 & 65.80 & 79.14 & 74.10 & \\
CLIP${^*}$ \cite{?}  & & & & & & & & & \\
Flamingo${^*}$ \cite{?}  & 68.15 & 81.89 & 80.20 & 73.10 & 77.35 & 81.86 & 78.48 & 77.09 & \\ \hline
\end{tabular}
\caption{\zhiwu{${^*}$indicates the corresponding model is fine-tuned on our database with any specific changes? It is better to report the results of ID and OOD (i.e., the test over Imagen and Parti) separately. It seems Flamigo has clearly better acc (AA) for OOD.} Results of the benchmark evaluation. Personalized Diffusion FT: fine-tuning, PT: prompt-tuning, AA: average detection accuracy, mAP: mean average precision. \textbf{Bold}: \textbf{best}, \underline{Underline}: \underline{second best}}
\label{tab:identification}
\end{table}




\begin{table}
\centering
\begin{tabular}{llll} 
\hline
Methods     & Num of Classes & F1-score & AC  \\ 
\hline
ViT        & 55        & 0        & 46.43    \\
Flamingo-ft & 55        & 0        & 45.20    \\
\hline
\end{tabular}
\caption{\zhiwu{Num of Classes is 55 or 3424+ reported in Table 2? We are expected to add  the results of ResNet and CLIP here like Table 4.} Results of identification. Personalized Diffusion}
\label{tab:identification}
\end{table}





\begin{table}
\centering
\begin{tabular}{llll} 
\hline
Methods     & CLIP Score & LPIPS & Avg  \\ 
\hline
BLIP        & 0.6508        & 0.6741       & 0    \\
Flamingo-ft & 0.6534   & 0.7034        & 0    \\
\hline
\end{tabular}
\caption{\zhiwu{The CLIP scores seem very close. Do we have any alternative metrics to measure the semantic similarity?} Results of prompt generation. }
\label{tab:prompt}
\end{table}









